MProtect: Operating System Memory Management without Access

Modern operating systems (OSes) have unfettered access to application data, assuming that applications trust them. This assumption, however, is problematic under many scenarios where either the OS provider is not trustworthy or the OS can be compromised due to its large attack surface. Our investigation began with the hypothesis that unfettered access to memory is not fundamentally necessary for the OS to perform its own job, including managing the memory. The result is a system called MProtect that leverages a small piece of software running at a higher privilege level than the OS. MProtect protects the entire user space of a process, requires only a small modification to the OS, and supports major architectures such as ARM, x86 and RISC-V. Unlike prior works that resorted to nested virtualization, which is often undesirable in mobile and embedded systems, MProtect mediates how the OS accesses the memory and handles exceptions. We report an implementation of MProtect called MGuard with ARMv8/Linux and evaluate its performance with both macro and microbenchmarks. We show MGuard has a runtime TCB 2~3 times smaller than related systems and enjoys competitive performance while supporting legitimate OS access to the user space.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> adaptation.tex <==
% !TEX root = ./main.tex
\subsection{App Binary Adaptation}
\label{sec:adaptation}

The \adp prepares an app binary for launching into a \secure process in an untrusted environment.
\name considers all loadable segments as sensitive and guarantees their confidentiality and integrity.

The \adp generates two symmetric keys and uses them to encrypt then sign the loadable segments.
It further encrypts the symmetric keys with the \tcb's public key and embeds the encrypted keys into the binary.

The \adp adds the following new segments into the binary, and modifies the entry point in binary header to \code{start} in the \shim.
\begin{itemize}[topsep=0.3em,itemsep=0.02em, leftmargin=*]

\item The \code{signature} segment contains signatures of the loadable segments.
The \tcb uses these signatures to check the integrity of the corresponding segments.

\item The \shim contains two trampolines into the \tcb: \code{start} and \code{resume}.
The \adp sets the entry point in binary header pointing to \code{start} so that the \tcb intervenes when a \secure process starts to run (\S\ref{sec:initialization}).
The \code{resume} trampoline is for resuming execution of a sensitive process after returning from an exception (\S\ref{sec:secure_exception_handle}).

\item The \code{metadata} segment contains metadata used by the \tcb during sensitive process initialization (\S\ref{sec:initialization}).
It includes a copy of program headers, original entry point, encrypted symmetric keys, and the signature of the above data, signed with the \adp's private key.

\item The \adp further reserves a memory areas as a \code{bss} segment to store signatures generated at runtime.
\end{itemize}

==> architecture.tex <==
\begin{table*}[!htbp]
\caption{Popular modern architectures support the architectural requirements of \name.}
\label{tab:arch_req}
\centering
\small
\begin{tabular}{|c | l | l | l|} 
\hline
Requirement & x86 & ARM & RISC-V\\\hline\hline
R1 & Hypervisor mode & Hypervisor and monitor modes & Machine mode \\
R2 & VM control structure (VMCS) & TVM in \code{hcr} register & TVM in \code{mstatus} register  \\
R3 & Hypervisor call (\code{vmcall}) & Trap of control register (e.g., \code{ctr}) access & Environment call (\code{ecall}) \\
\hline
\end{tabular}
\end{table*}

\design has three requirements for the architectures:
\begin{enumerate}[topsep=0.3em,itemsep=0.02em, leftmargin=*, label=\textit{A\arabic*.}]
    \item A programmable privilege mode higher than what the OS is running in.
    \item A way to trap updates of the virtual memory control registers into the higher privilege mode.
    \item A mechanism with which an application can invoke the higher privileged software, bypassing the OS.
\end{enumerate}
x86, ARM and RISC-V all meet these requirements as shown in Table~\ref{tab:arch_req}.
We note that Nested kernel~\cite{dautenhahn2015nested} provides a \emph{software} alternative in which the nested kernel has a higher privilege than the outer kernel (\textit{R1}).
The nested kernel de-privileges the outer kernel via scanning its code to ensure no instruction updating virtual memory control registers (\textit{R2}) and an application can invoke the nested kernel with normal system call bypassing the outer kernel (\textit{R3}).

==> initialization.tex <==
\section{\Secure Process Creation}
\label{sec:initialization}

By the time the OS is about to start running an app, it has already set up the user page table and mapped loadable segments of the binary to the user address space, unaware that all the loadable segments are encrypted.  
When the OS transfers control to the entry point of the app, it unknowingly invokes the \code{start} trampoline and traps into the \tcb.

When the \tcb takes over, it first hides frames hosting the \code{metadata} segment from the OS, i.e., invalidating the corresponding kernel page table entries.
It then checks the integrity of the data with the \adp's public key and extracts the symmetric keys with its own private key.
\lin{Lin's note: adapter's public key to developer's public key.}

With the metadata, the \tcb parses the program headers and walks the list of virtual memory area descriptors in the kernel space to learn the virtual addresses of other segments. It then walks the user page table. If a page is present, the \tcb hides the mapped frame from the OS, checks its integrity and decrypts its content with the extracted keys.

The \tcb also triggers the OS to create the \shadow page table via faking a page fault (see \S\ref{sec:context_fault}).
Finally, the \tcb configures the vector base address register (\code{VBAR}) to the address of the secure \exvec (see \S\ref{sec:context_switch}) and returns control to the original entry point. From then on, the sensitive process is under runtime protection from the \tcb.

To protect sensitive processes, the \tcb identifies a process by the base address of its page table.
Likewise, we use the value of the stack pointer (SP) to identify threads within a \secure process.
Notably, the \tcb does not trust the unique process identifier (PID) assigned to each process by Unix-like OSes. 
